Navigating Threats: A Survey of Physical Adversarial Attacks on LiDAR Perception Systems in Autonomous Vehicles

Autonomous vehicles (AVs) rely heavily on LiDAR (Light Detection and Ranging) systems for accurate perception and navigation, providing high-resolution 3D environmental data that is crucial for object detection and classification. However, LiDAR systems are vulnerable to adversarial attacks, which pose significant challenges to the safety and robustness of AVs. This survey presents a thorough review of the current research landscape on physical adversarial attacks targeting LiDAR-based perception systems, covering both single-modality and multi-modality contexts. We categorize and analyze various attack types, including spoofing and physical adversarial object attacks, detailing their methodologies, impacts, and potential real-world implications. Through detailed case studies and analyses, we identify critical challenges and highlight gaps in existing attacks for LiDAR-based systems. Additionally, we propose future research directions to enhance the security and resilience of these systems, ultimately contributing to the safer deployment of autonomous vehicles.

==> draft.tex <==
Attacks on 3D Object Detection:

LiDAR-Based.

MMF-Based.

==> draft_constraint.tex <==
% \label{techniques}

\section{Challenges and Physical Constraints}

\subsection{Attacks on Images vs. Point Clouds}

Attacking images and point clouds involves distinct challenges due to their differing data structures and attack methodologies.

%\textbf{Different perturbation methods.} Images and point clouds have different data structures, which further lead to different perturbation methods applied. Images have compact and ordered structures. In contrast, point clouds are irregular, represented as $N \times C$, where N is the number of points, and C contains the location and intensity information (i.e., xyz-i) \cite{kitti}. Attackers are able to generate adversarial examples by modifying the RGB values in images. For attacks on LiDAR, however, attackers can directly shift the point in the 3D Euclidean space as long as it obeys the physics of LiDAR.
\noindent\textbf{Different Perturbation Methods.}
Images and point clouds have fundamentally different data structures, leading to unique perturbation methods. Images are compact and ordered, while point clouds are irregular, represented as $N \times C$, where $N$ is the number of points and $C$ contains location and intensity information. In image-based attacks, adversaries can manipulate the RGB values to generate adversarial examples. However, in LiDAR-based attacks, adversaries manipulate the points directly in 3D Euclidean space, ensuring that the perturbations comply with the physical constraints of LiDAR.

% \noindent\textbf{Different perturbation capabilities.} Prior attacks on 2D images treat the whole target area as the attack surface since the threat model assumes that attackers have full controls over the target object (e.g., attackers can potentially modify any area of a stop sign in \cite{eykholt2018robust}). However, due to the characteristics of LiDAR spoofing attacks, the attack surface is limited by the sensor attack capability (A). Such a small attack surface also introduces difﬁculties in launching the attack.
\noindent\textbf{Different Perturbation Capabilities.}
In 2D image attacks, the entire target area can often serve as the attack surface, assuming that attackers have full control over the object (e.g., attackers can alter any part of a stop sign, as shown in \cite{eykholt2018robust}). However, in LiDAR spoofing attacks, the attack surface is significantly constrained by the sensor’s physical capabilities. This smaller attack surface introduces additional challenges, making it harder to execute successful attacks on point clouds.

% \noindent\textbf{Different perturbation constraints.} Prior attacks on 2D images leverage Lp norms as the main constraints for the formulated optimization problem \cite{eykholt2018robust} whose goal is to minimize the perturbation to be stealthy. Such constraints do not apply to attack LiDAR because point clouds are not perceived by humans. Thus, stealthiness is not a focus in such attacks. Instead, the optimized attack traces must not exceed the sensor attack capability (A) boundary, in which case A naturally becomes the primary constraint for attacking LiDAR.
\noindent\textbf{Different Perturbation Constraints.}
In image-based attacks, Lp norms are commonly used to constrain the perturbations during optimization, with the goal of making the perturbations as imperceptible as possible \cite{eykholt2018robust}. These constraints do not apply to LiDAR attacks because point clouds are not visually perceived by humans, making stealthiness less of a priority. Instead, the primary constraint in LiDAR attacks is ensuring that the adversarial perturbations remain within the sensor's physical capabilities, which becomes the defining limitation for the attack.

%Second, the high-level methodology of our proposed attack is similar to replay attacks, in which adversaries playback the intercepted data to deceive target systems [11]. However, different from existing replay attacks [44] that re-transmit logically correct data to launch attacks, the limited sensor attack capability (A) cannot support the injection of a physically valid vehicle’s trace into the LiDAR point cloud [17]. Thus, the success of our black-box attack indeed relies on the identified vulnerability.

% \textbf{Physical Constraint for Spoofing Attack}\\
\subsection{Spoofing Attacks}

% \subsubsection{For Object Injection}
% The point cloud space is sparse. Every generated point can only reside on one of the sparse LiDAR’s laser rays, and each laser ray can record at most one point. Therefore, to ensure that the LiDARs can perceive adversarial points emitted by the adversary’s transmitter in the real world, we must ensure that the added adversarial points align with these laser rays. Specifically, we adhere to the following physical constraints when generating adversarial points:

% \textbf{(*) Each laser ray can record at most one point.} Autonomous vehicles equipped with LiDARs often operate under the Strongest Return Mode setting \cite{cao2019ccs}. In this mode, each laser only records the point with the highest reflection intensity. Without proper constraints on the adversarial points, there might arise a situation where two adversarial points appear on the same laser ray, violating physical reality.

% \textbf{(**) The vertical angles of the adversarial points must align with the laser ray’s discrete specific angles.} Common mechanical LiDARs used in AD come in configurations like 16-line, 32-line, 64-line, and so on (refer to Fig. \ref{fig:lidar}). These laser beams are distributed at specific vertical angles centered on the LiDAR. As a result, it’s crucial to ensure that the added adversarial points fall within these preset angles. 

% \textbf{(***) The horizontal angle of the adversarial points must be restricted to a narrow range.} The attacker’s capabilities are bound by hardware constraints, such as the laser transmitter. As such, it’s infeasible to inject adversarial points across the full 360° horizontal angle of the target LiDAR simultaneously. Currently, attackers can generally introduce adversarial points within a 10° horizontal angle distribution.
%-----------------------------------
\subsubsection{Object Injection Constraints}
%-----------------------------------
The point cloud generated by a LiDAR sensor is inherently sparse, as each laser ray can capture at most one point. To ensure that adversarial points emitted by an attacker’s transmitter are successfully perceived by the LiDAR in a real-world setting, it is crucial that these points align with the sensor’s laser rays. The following physical constraints must be adhered to when generating adversarial points:

\begin{itemize}
    \item \textbf{Each laser ray can record at most one point:} Most autonomous vehicles equipped with LiDARs operate in the Strongest Return Mode \cite{cao2019ccs}, where each laser records only the point with the highest reflection intensity. Without proper alignment of adversarial points, multiple points may be generated on the same laser ray, which would violate the physical behavior of the LiDAR system.
    \item Vertical alignment with discrete laser angles: Mechanical LiDARs commonly used in autonomous driving (AD) feature specific configurations, such as 16-line, 32-line, or 64-line setups (as illustrated in Fig. \ref{fig:lidar}). These beams are distributed at distinct vertical angles relative to the LiDAR. Therefore, adversarial points must be placed at the discrete vertical angles corresponding to these preset beams.
    \item \textbf{Horizontal angle constraints:} The adversary’s ability to inject points is constrained by the limitations of their hardware, such as the laser transmitter. Injecting adversarial points across the entire 360° horizontal field of view of the LiDAR is not feasible. Current attack methods can typically introduce adversarial points within a limited 10° horizontal angle range.
\end{itemize}
 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/lidar.png}
    \caption{Velodyne HDL-64E has 64 lasers, and their vertical angle range is -24.8° to 2°. 32 lasers in lower laser block separated by 1/2° vertical spacing and 32 lasers in upper laser block separated by 1/3° vertical spacing. (Figure adapted from \cite{yang2023}).}
    \label{fig:lidar}
\end{figure}

\cite{cao2023}

% \subsubsection{For Object Removal}
% The removal attack capability is limited by two factors: 
% \textbf{(*) the limited receptive field of the photodiodes of the LiDAR system.} This constrain is due to the optical components inside the LiDAR only receiving reflections from certain directions. Therefore, when the spoofer is out of the receptive range, the spoofed signals are not received by the LiDAR system, so the removal attack fails. \\
% \textbf{(**) the limited output power of the laser diodes in our single-spoofer setup.}  The limited output power of the laser diodes generate a diverged circular laser spot, even with the optical support to converge it. The intensity of the spoofed pulses are lower when they get nearer to the edge of the spot. When the signal is too weak to spoof the points, the removal attack fails. Also, due to the decaying intensity as the distance between the spoofer and the LiDAR increases, the removal attack capability also decreases. Many of these limitations are therefore caused by the spoofer design.
%-----------------------------------
\subsubsection{Object Removal Constraints}
%-----------------------------------
The effectiveness of object removal attacks is constrained by two key factors:

\begin{itemize}
    \item \textbf{Limited receptive field of the LiDAR’s photodiodes:} The optical components of a LiDAR system are designed to receive reflections only from certain directions within a specific range. If the spoofer is positioned outside of this receptive field, the LiDAR is unable to detect the spoofed signals, leading to the failure of the removal attack.
    \item \textbf{Limited output power of the laser diodes in a single-spoofer setup:} The laser diodes in the spoofer have restricted output power, which results in the laser beam spreading into a diverging circular spot, even when optical components are used to focus it. As the spot extends outward, the intensity of the spoofed pulses diminishes, particularly near the edges of the spot. When the signal becomes too weak, the LiDAR fails to register the spoofed points, causing the removal attack to be ineffective. Additionally, as the distance between the spoofer and the LiDAR increases, the intensity of the spoofed signal further decays, reducing the overall effectiveness of the attack. Many of these limitations stem from the design of the spoofer itself.
\end{itemize}


\subsection{Physical Object-based Attacks}

% \textbf{Techniques for Turning Adversarial Points into Physical Objects.}

Turning the generated point cloud that can achieve adversarial effects into adversarial objects is not trivial to transfer these “virtual points” into real road conditions.

\subsubsection{Technique 1: Targets only LiDAR (Shape only)}

% \cite{tsai2020robust} does that through surface reconstruction from adversarial point cloud data. The uncertainty in the reconstruction process weaken the attack success rate in real world environment. They also fail to consider the mechanism of specific type of sensors and simply apply random sampling to simulate the 3D sensors.
% \cite{yang2021} creating physical objects in the beginning of attack that appear as adversarial point clouds when scanned by Lidar. first simulate the working process of Lidar sensors. The simulation tool creates a point cloud from a scene based on 3D meshes. Adding a list of models and the scene builder script easily creates random distributions of objects. The Lidar script creates point clouds from these scenes by ray tracing. By setting the parameter according to the configuration, the simulation tool internally creates a set of rays, whose intersections with a given 3D object are then calculated, returning a series of 3D coordinates of point cloud. The difference in the angle between the rays can be specified during initialization of the Lidar class, as well as the position of the Lidar sensor. Specifically, for the Lidar simulation process, the following parameters should be given: 

% \begin{itemize}
%     \item Lidar parameters, such as position $R = (r_x, r_y, r_z)$ azimuth resolution, etc.
%     \item Object information including vertices $v \in \mathbb{R}^{n\times3}$ and polyhedrons $p \in \mathbb{N}^{m\times3}$.
% \end{itemize}

% In \cite{yang2021}, choose to modify the object vertices $v$ by adding certainly designed perturbations $\delta$, and leave other information untouched. To simulate different viewing angles and distances, they randomly place the LiDAR at different pre-defined positions. Given the objects and the Lidar parameters, the simulation process:

% \begin{itemize}
%     \item Line-plane intersection: Determine the intersection between the rays and the object surfaces.
%     \item Point in polygon: Check whether there is any polygon, i.e., surface, that the point is inside of it.
%     \item Distance comparison: Filter out the points belonging to the polygons that are obstructed by other obstacles.
% \end{itemize}

% Given a set of polygons (represented by triangles in 3D space) and Lidar rays (represented by lines in 3D space), the points captured by Lidar can be calculated by intersecting the lines with the polygons. Considering a polygon $p_i = \{v_0, v_1, v_2 | v_i \in \mathbb{R}^3\}$ and a ray denoted by its origin
% $R = (r_x, r_y, r_z)$ and direction $D_i = (d_x, d_y, d_z)$, they first let 
% $n = (n_x, n_y, n_z)$ be the normal vector of the polygon $p_i$. The point $x_i \in \mathbb{R}^3$ can then be given by:

% \begin{equation}
%     x_i = R + D_i \times \frac{(v_0 - R)\cdot n}{D_i \cdot n}
% \end{equation}

% Since this process is differentiable, they can integrate this procedure into their optimization problem, so that it can be solved directly using existing mechanisms. In practice, the gradients can be automatically calculated within most of the deep learning frameworks including TensorFlow and PyTorch.
% After the line-plane intersection, points that are either obstructed by other obstacles or not located inside the polygons will be filtered out. The remaining points are the input to the PointRCNN.

Tsai et al. \cite{tsai2020robust} tackle the problem by reconstructing surfaces from adversarial point cloud data. However, the inherent uncertainty in the reconstruction process reduces the attack success rate in real-world environments. Additionally, their approach overlooks the specific mechanisms of various sensor types, instead relying on random sampling to simulate 3D sensors, which limits the accuracy of the simulation.

In \cite{yang2021}, the authors create physical objects at the beginning of the attack that, when scanned by LiDAR, appear as adversarial point clouds. Their method first simulates the operational process of LiDAR sensors by generating a point cloud from a scene built using 3D meshes. The simulation tool allows for the easy inclusion of models and scene-building scripts to create random object distributions. Using ray tracing, the tool generates point clouds by calculating intersections between LiDAR rays and objects. The parameters of the LiDAR, such as azimuth resolution and position, can be adjusted during initialization, allowing for accurate simulation of the sensor's configuration. Specifically, the following parameters are required for the LiDAR simulation process:

\begin{itemize}
    \item LiDAR parameters, including its position $R = (r_x, r_y, r_z)$, azimuth resolution, and other relevant settings.
    \item Object information, such as vertices $v \in \mathbb{R}^{n\times3}$ and polyhedrons $p \in \mathbb{N}^{m\times3}$.
\end{itemize}

In \cite{yang2021}, the vertices of the objects, $v$, are modified by adding carefully crafted perturbations $\delta$, while other object attributes remain unchanged. To simulate various viewing angles and distances, the LiDAR is randomly placed at predefined positions around the objects. Given the objects and LiDAR parameters, the simulation process consists of the following steps:

\begin{itemize}
    \item \textbf{Line-plane intersection}: Calculate the intersections between LiDAR rays and the surfaces of the objects.
    \item \textbf{Point-in-polygon check}: Verify whether the intersection points lie within the object’s polygons (surfaces).
    \item \textbf{Distance comparison}: Exclude points that belong to polygons obstructed by other obstacles.
\end{itemize}

To determine the points captured by the LiDAR, the simulation calculates the intersection between LiDAR rays and 3D polygons (represented as triangles). Given a polygon $p_i = \{v_0, v_1, v_2 | v_i \in \mathbb{R}^3\}$ and a ray originating from $R = (r_x, r_y, r_z)$ with direction $D_i = (d_x, d_y, d_z)$, the normal vector of the polygon is denoted as $n = (n_x, n_y, n_z)$. The intersection point $x_i \in \mathbb{R}^3$ is then calculated using the equation:

\begin{equation}
    x_i = R + D_i \times \frac{(v_0 - R)\cdot n}{D_i \cdot n}
\end{equation}

Since this process is differentiable, it can be integrated into an optimization framework, allowing it to be solved directly using existing techniques. Gradient calculations can be handled automatically by deep learning frameworks such as TensorFlow and PyTorch. After performing the line-plane intersection, points that are either obstructed or fall outside the polygons are filtered out. The remaining points serve as the input for the PointRCNN model.

% \noindent\textbf{Physical Printing Constraints.}
% to realize these objects into a real road environment, we need to consider many physical constraints. Considering the volume of popular 3D printer, we limit the size of adversarial objects to 45cm × 45cm × 41cm, which is much smaller comparing to common vehicles or pedestrians. We also force a large plane on the bottom of the object so that the object can easily support itself.

% In \cite{yang2021}, Since our target is to generate an object that can mislead the model, the “dis-similarity” between the original one and the modified one is not a critical concern. That is, the object we generate do not have to be similar to the original one in our attack settings. Thus, the distance constraints, such as $L_2$ norm or Chamfer distance, will not be considered in our objective function to obtain more flexibility in forming the shape of adversarial objects.

% Instead of adding another term to objective function, we directly decrease the perturbations to make sure that the length of each axis will not exceed the pre-defined threshold. For example, if the length of the object in $x$ axis is greater than the threshold $l_x$, the following action will be applied to enforce the size limit.
\noindent\textbf{Physical Printing Constraints:}
To deploy these adversarial objects in a real road environment, several physical constraints must be considered. Due to the volume limitations of commonly available 3D printers, we restrict the size of adversarial objects to 45 cm × 45 cm × 41 cm, which is considerably smaller than typical vehicles or pedestrians. Additionally, we design a large, flat surface at the base of the object to ensure structural stability, allowing it to support itself effectively.

In \cite{yang2021}, since the primary goal is to generate an object that misleads the model, the “dissimilarity” between the original object and the modified version is not a significant concern. In this attack setting, the adversarial object does not need to closely resemble the original one. Consequently, distance metrics such as the $L_2$ norm or Chamfer distance are not considered in the objective function, providing more flexibility in shaping the adversarial object.

Instead of incorporating additional terms into the objective function, we directly reduce the perturbations to ensure that the object’s dimensions stay within predefined limits. For example, if the length of the object along the $x$-axis exceeds the threshold $l_x$, adjustments are made to enforce the size constraint.
%----------------------------------------------------------------------
\subsubsection{Technique 2: Targets LiDAR and Camera (Shape and Texture)}
%----------------------------------------------------------------------

% Abdelfattah et al. \cite{abdelfattah2021}

% To make a realistic adversarial attack on multi-modal DNNs that can target both camera and LiDAR modalities, we require a representation that can maintain realistic 3D physical geometry and also can be differentiably rendered to RGB images and LiDAR. We choose a mesh for our adversarial object, since it provides an efﬁcient representation of a 3D object and can be rendered to images or point clouds. This adversarial mesh is placed on top of a vehicle to avoid occlusion, and rotated around the vertical axis to have the same orientation as the vehicle. To train the shape of the object, following previous work \cite{cao2019adversarial, tu2020}, we start with an initial mesh $S$ with $V$ vertices, where each initial vertex is deﬁned as $v^0_i \in \mathbb{R}^3~, i \in \{1,2,\dots,V\}$. We deform the shape of the mesh by displacing each vertex with a displacement vetcor $\hat{v}_i \in \mathbb{R}^3$, which is a learnable parameter to produce an adversarial mesh $S^{adv}$ with vertices $v_i$'s, as in Equation \ref{abd21}. We use $4 \times 4$ transformation matrix $T$ to put the mesh on top of a car and give it the same orientation:

% \begin{equation}
%     \label{abd21}
%     v_i = T \cdot (v^0_i + \hat{v}_i)
% \end{equation}
% For the texture of the adversarial mesh, we give each vertex a corresponding RGB color $c^i \in \mathbb{R}^3$, which is a learnable parameter. We then render the mesh to 2D and add it to the original RGB scene using a given projection matrix. To produce the texture of the mesh, each face is colored by the interpolation of the colors from the vertices surrounding it. 

% To ensure our object is realistic, we put constraints on the size and smoothness of the mesh geometry. Also since we interpolate between vertex colors to produce the adversarial texture, the result is a realistic smooth texture without abrupt changes in color (a typical observation in RGB adversarial attacks using pixel-wise perturbations).
To execute a realistic adversarial attack on multi-modal deep neural networks (DNNs) that target both camera and LiDAR modalities, we require a representation that preserves realistic 3D physical geometry and can be differentiably rendered into both RGB images and LiDAR point clouds. They opt for a mesh representation for the adversarial object, as it provides an efficient and flexible 3D structure that can be rendered into images or point clouds. This adversarial mesh is positioned on top of a vehicle to avoid occlusion and is rotated around the vertical axis to align with the vehicle’s orientation.

To train the shape of the object, we follow the approach of previous works \cite{cao2019adversarial, tu2020}. Starting with an initial mesh $S$ composed of $V$ vertices, each initial vertex is defined as $v^0_i \in \mathbb{R}^3$, where $i \in {1,2,\dots,V}$. They deform the mesh by applying a displacement vector $\hat{v}_i \in \mathbb{R}^3$ to each vertex. This vector is a learnable parameter that generates the adversarial mesh $S^{adv}$ with the modified vertices $v_i$, as described in Equation \ref{abd21}. The mesh is then placed on top of the vehicle and oriented using a $4 \times 4$ transformation matrix $T$:

\begin{equation} \label{abd21} v_i = T \cdot (v^0_i + \hat{v}_i) \end{equation}

For the texture of the adversarial mesh, we assign each vertex a corresponding RGB color $c^i \in \mathbb{R}^3$, which is also a learnable parameter. The mesh is then rendered into 2D and integrated into the original RGB scene using a projection matrix. The texture of the mesh is determined by interpolating the colors of the surrounding vertices, ensuring smooth transitions across the faces.

To ensure the object remains realistic, we impose constraints on the size and smoothness of the mesh geometry. Since we generate the adversarial texture by interpolating between vertex colors, the resulting texture is smooth and natural, avoiding abrupt color changes that are typically observed in RGB adversarial attacks using pixel-wise perturbations.

% \noindent\textbf{Differentiable Rendering}
% To realistically render a mesh to point cloud, we need to ﬁnd which LiDAR rays would intersect with the mesh if it was placed in the original scene. We simulate the LiDAR used in capturing the dataset’s point cloud by producing rays at the same angular frequencies and incorporating a small amount of noise that is present in this speciﬁc LiDAR. We then calculate the intersection points between these rays and our mesh’s triangles in the 3D scene using the M\"oller–Trumbore intersection algorithm \cite{moller2005fast}. Finally, for each ray with intersection points we take the nearest point, and add all the resulting points to the LiDAR point cloud scene.
% After placing our mesh on top of all cars in a 3D scene, we render the meshes to 2D using a given projection matrix. To train our adversarial texture, the rendering process needs to be differentiable. We therefore use the fast, differentiable rendering tools developed in \cite{johnson2020accelerating} to render our adversarial mesh from the 3D scene to RGB images, as shown in Figure \ref{fig:abdelfattah2021}.
%-------------------------------------------
\noindent\textbf{Differentiable Rendering:}
%-------------------------------------------
To realistically render a mesh into a point cloud, they need to determine which LiDAR rays would intersect with the mesh when placed in the original scene. To achieve this, they simulate the LiDAR used to capture the dataset’s point cloud by generating rays at the same angular frequencies and adding a small amount of noise to reflect the inherent noise in the specific LiDAR system. They then calculate the intersection points between these rays and the triangles of our mesh in the 3D scene using the Möller–Trumbore intersection algorithm \cite{moller2005fast}. For each ray that intersects with the mesh, they select the nearest intersection point and add it to the LiDAR point cloud of the scene.

Once the mesh is positioned on top of all vehicles in the 3D scene, they render it into 2D using a projection matrix. To optimize the adversarial texture, the rendering process must be differentiable. Therefore, they employ fast, differentiable rendering tools as developed in \cite{johnson2020accelerating} to render our adversarial mesh from the 3D scene into RGB images, as illustrated in Figure \ref{fig:abdelfattah2021}.

% \noindent\textbf{Physical Printing Constraints.}
% We ﬁrst perturb the geometry of the object, to attack the 3D part. We start with a 40 cm radius isotropic sphere mesh with 162 vertices and 320 faces. We apply box constraints to keep the mesh’s 3 dimensions below the initial levels.
% We apply box constraints to keep the mesh’s 3 dimensions below the initial levels. An ADAM optimizer is then used to iteratively deform the mesh to minimize (3). Once we have an adversarial shape we render it to 2D images and train a universal adversarial texture. We give each vertex an initial color and then we use an ADAM optimizer to learn which color, for each vertex, would produce an adversarial texture to attack the RGB pipeline.
%-------------------------------------------
\noindent\textbf{Physical Printing Constraints:}
%-------------------------------------------
To initiate the attack on the 3D model, they first perturb the geometry of the object. They begin with an isotropic sphere mesh with a 40 cm radius, consisting of 162 vertices and 320 faces. Box constraints are applied to ensure that the mesh’s dimensions remain within their initial bounds throughout the deformation process.mUsing the ADAM optimizer, they iteratively deform the mesh to minimize the attack objective function. Once the adversarial shape is generated, it is rendered into 2D images to facilitate the training of a universal adversarial texture. Each vertex is initially assigned a color, and the ADAM optimizer is then employed to learn the optimal color for each vertex that produces an adversarial texture, effectively targeting the RGB pipeline.

%======================================
\subsubsection{Design Challenges Multi-Sensor Based Perception}
%=======================================
\cite{cao2021}

\noindent\textbf{Design a single physical-world attack vector effective for both camera- and LiDAR-based AD perception.}
To achieve the attack goal, we need to ﬁnd physical-world attack vectors for both camera- and LiDAR-based perception networks in MMF. For camera-based AD perception, previous works predominately consider adding stickers/posters \cite{song2018physical, zhao2019seeing}, painting \cite{zhang2019camou, chen2019shapeshifter}, or changing brightness \cite{pei2017deepxplore, tian2018deeptest}, which can only change the texture of an obstacle but not its shape and thus can barely affect the LiDAR point clouds. On the LiDAR side, LiDAR spooﬁng \cite{cao2019ccs, sun2020}, which shoots lasers to LiDAR, has shown to be effective in the AD context. Although lasers can also affect camera inputs \cite{yan2016can}, no prior work has studied its effectiveness for fooling camera-based AD perception models. One possible solution is to use separate attack vectors for them, e.g., using stickers for camera and laser shooting for LiDAR. However, this not only adds up the attack deployment costs and thus lowers the realizability and stealthiness, but also requires precise synchronizations across the attack processes. Thus, it is highly desired to identify one single attack vector that can effectively attack both at the same time.


\noindent\textbf{Need to differentiably synthesize physically-consistent attack impacts onto both camera and LiDAR.}
To systematically generate adversarial inputs, prior works generally adopt optimization-based approaches, which have shown both high efﬁciency and effectiveness \cite{zhao2019seeing, athalye2018synthesizing}. Since adversarial attack generation typically takes thousands of optimization iterations \cite{madry2017towards, carlini2017towards}, it is almost impossible in practice to physically drive vehicles on the target road to obtain the attack-inﬂuenced camera images and LiDAR point clouds every time the adversarial inputs are updated in an iteration. Thus, we need to digitally synthesize the impacts of the adversarial stimulus from the physical world onto both camera images and LiDAR point clouds, and such synthesizing needs to be differentiable to enable effective optimization.


\noindent\textbf{Need to handle non-differentiable pre-processing steps in AD perception.}
In industry AD systems, images and point clouds are usually pre-processed before fed into the MMF algorithm. In particular, state-of-the-art LiDAR-based AD perception models popularly use aggregated features of 3D points grouped at level of 2D or 3D cells. To calculate such cell-level aggregated features, the necessary ﬁrst step is to calculate whether an input point is inside a cell or not. In this paper, we call it a point-inclusion property. By nature, such property is discontinuous, i.e., 0 and 1 for outside and inside a cell. This causes the calculation of any cell-level aggregated features non-differentiable with regard to the LiDAR point clouds, which thus makes our optimization difﬁcult to be effective. So far, no prior works have considered a general design to handle such non-differentiable pre-processing steps for LiDAR.

==> taxonomy_draft.tex <==
\section{TAXONOMY OF ADVERSARIAL ATTACKS}
We present our taxonomy of adversarial attacks for object detection in Figure \ref{fig:taxonomy}. We describe preliminary information in Section \ref{preliminaries}, followed by detailed categorizations for attack model and attack method in Section \ref{model} and \ref{method}, respectively.

\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{Figures/taxonomy.png}
    \caption{Taxonomy and evaluation metrics on adversarial attacks for 3D object detection.}
    \label{fig:taxonomy}
\end{figure*}

\subsection{Preliminaries}
\label{preliminaries}
% \subsubsection{Point-wise perturbation}
\cite{cai2020}
Given the input scene point cloud $S$ and the ground truth location $G$ of the target objects %belonging to $C$
, the point cloud $X= \{x_i\}^{N'}_{i=1}$ of a target can be obtained, satisfying $X \in S$. We apply point-wise perturbations to the target point cloud $X$, and generate adversarial point clouds to attack a deep $3D$ object detection model.

Denote $\{\delta_i\}^{N'}_{i=1}$ as the perturbation vectors, satisfying $\delta_i \in \mathbb{R}^3$, added to the point cloud of the target $X$, producing adversarial point cloud $X'= \{x_i + \delta_i\}^{N'}_{i=1}$. A target proposal $p_i$ generated by a deep $3D$ object detection model can be called positive, if its Intersection of Union (IoU) with ground truth bounding box of a corresponding object is larger than a threshold $\mu$ and at the same time its confidence score is greater than a threshold $\alpha$. The others are defines as negative. 

The adversarial attack can be formulated as an unconstrained optimization problem, and the loss function are defined as follows:

\begin{equation}
    L = L_{adv} + \lambda L_{per},
\end{equation}

where $L_{adv}$ and $L_{per}$ stand for the corresponding adversarial loss and point cloud perturbation loss, and $\lambda$ is used as a weighing parameter.

The adversarial loss $L_{adv}$ is defined on the whole set of positive proposals, and is designed to minimize both their Intersection of Union with the ground truth and the associated confidence, as follows:

\begin{equation}
    L_{adv} = \sum_{(p_i, s_i)\in P} -IoU(p_i,p^*)log(1-s_i),
\end{equation}

where $P$ represents the whole set of positive target proposals with $p_i$, $s_i$ standing for the $i$th bounding box and the associated confidence. $p^*$ is denoted as the ground truth of the bounding box. The operator $IoU(\dot,\dot)$ calculates the intersection between two bounding boxes.

To make sure that the generated adversarial point cloud is visually imperceptible to humans, the perturbation loss $L_{per}$ is added. A number of distance metrics have been proposed to measure the deviation of the adversarial point clouds from the origin, such as Hausdorff distance, chamfer distance. In this paper, we choose the $L_2$ norm distance for its efficiency both in performance and computation. Thus given the target point cloud $X$, the perturbation vectors $\{\delta_i\}^{N'}_{i=1}$, and the adversarial point cloud $X'= \{x_i + \delta_i\}^{N'}_{i=1}$, the perturbation loss $L_{per}$ can be defined as follows:

\begin{equation}
    L_{per} = \sum^{N'}_{i=1}\parallel\delta_i\parallel^2.
\end{equation}

To sum up, the loss function defined for the adversarial attack is defined as follows:

\begin{equation}
    L_{adv} = \sum_{(p_i, s_i)\in P} -IoU(p_i,p^*)log(1-s_i) + \lambda\sum^{N'}_{i=1}\parallel\delta_i\parallel^2.
\end{equation}

Given the loss function defined on the point cloud perturbations, the adversarial attack can be realized by the means of differentiation. To be specific, the optimization process is guided by the gradient computed from the loss function with respect to each point. $\lambda$ defined in the loss function is set as a constant $0.1$. 



%%==============================================
\subsection{Attack Model}
%%==============================================
\label{model}

%%==============================================
\subsubsection{Attack Setting} %Environment
%%==============================================

\textbf{Digital}: Digital attacks involve altering the points of point clouds input into the target model without interacting with the physical environment. In this type of attack, the attacker manipulates the data directly within the digital realm, meaning they do not interfere with the actual physical objects or the environment being scanned. The attacker also lacks access to the processes of information capture, pre-processing, and post-processing, focusing solely on the digital manipulation of the input data to deceive the target model.

\noindent\textbf{Physical}: Physical attacks, on the other hand, involve direct manipulation of the physical environment or objects within the LiDAR sensor's field of view. In this scenario, the attacker alters real-world objects or settings in ways that affect how they are perceived by the LiDAR system. This could include placing reflective materials, altering the shape or surface of objects, or introducing new objects to the environment to create misleading or false data in the point cloud. Unlike digital attacks, physical attacks exploit the real-world conditions that the LiDAR sensor captures, aiming to disrupt the system’s ability to accurately detect and classify objects.
We focus on physical attacks in this literature review as they present more realistic and practical threats to autonomous vehicle systems, highlighting the importance of addressing these vulnerabilities to ensure the safety and reliability of autonomous driving technologies.
% \textcolor{red}{add specifications, things like techniques, pre-processing, post-processing modeling, synchronization}

%%==============================================
\subsubsection{Test Scenario}
%%==============================================

\textbf{Simulation}: Simulated attacks are performed within controlled, virtual environments where the entire system, including the LiDAR sensors and the physical environment, is modeled in software. This setting allows researchers and attackers to experiment with different attack techniques, pre-processing, post-processing, and synchronization challenges without the risks associated with real-world testing. Simulated environments enable precise control over the variables, making it easier to study the effects of various attack strategies and to refine them before potentially applying them in real-world scenarios. Common techniques in simulated attacks include generating synthetic point clouds that incorporate adversarial perturbations and testing the effects of these perturbations across different models and sensor configurations.

\noindent\textbf{Real-World}: Real-world attacks involve deploying adversarial techniques in actual environments where autonomous vehicles or LiDAR-equipped systems operate. These attacks are more challenging due to the complexities and unpredictability of real-world conditions, such as variable lighting, weather, and the dynamic nature of the environment. Real-world attacks require careful planning and execution, including synchronizing the timing of the attack with the vehicle’s sensors and considering the physical constraints of manipulating objects in a real environment. The attacker must also account for the entire sensor processing pipeline, from pre-processing (such as filtering noise from the point cloud) to post-processing (such as data fusion and decision-making algorithms), ensuring that the attack is effective across all stages. Real-world attacks are the most concerning as they pose direct threats to the safety and functionality of autonomous vehicles, making them a critical focus for defensive strategies.

%%==============================================
\subsubsection{Attacker Knowledge}
%%==============================================
% \textbf{System Level.}\\
% \textbf{White-box attacks}: White-box attacks: In a white-box attack, the adversary has complete knowledge of the target model. Information includes the model input and output, neural network architecture, parameter weights and gradients, decision making process, and training procedure and dataset. The attacker either has full access to the target model or has the capability to completely reconstruct the target model. With this level of information, the adversary can craft attacks specific to the target model.

% \noindent\textbf{Black-box attacks}: In a black-box attack, the adversary has no knowledge of the target model. The adversary may submit input queries and observe the predicted bounding boxes and class confidence scores. Common models and algorithms can be used as surrogates as they may share vulnerabilities with the target model.

% \noindent\textbf{Grey-box attacks}: partial knowledge

% \textbf{Environmental Level.}\\
% The attacker knows the approximate position of the target object so as to obtain a frustum region for spoof point placement. In addition to FP outcomes, this also enables FN or translation attack outcomes targeting a particular (valid) object.
\textbf{System Level.}\\
\textbf{White-box attacks}: In a white-box attack, the adversary possesses complete knowledge of the target model, including the input-output pairs, neural network architecture, parameter weights, gradients, decision-making process, training procedure, and dataset. The attacker either has direct access to the model or the ability to fully reconstruct it. With such comprehensive knowledge, the adversary can craft highly targeted attacks that exploit specific vulnerabilities of the model.

\noindent\textbf{Black-box attacks}: In a black-box attack, the adversary has no prior knowledge of the internal workings of the target model. They can only interact with the system by submitting input queries and observing the resulting outputs, such as predicted bounding boxes or class confidence scores. To mount an effective attack, the adversary may use surrogate models with similar vulnerabilities, leveraging these commonalities to find weaknesses in the target system.

\noindent\textbf{Grey-box attacks}: In a grey-box attack, the adversary has partial knowledge of the target system, such as some aspects of the model architecture or limited access to certain input-output pairs, but lacks full access to the complete model.

\noindent\textbf{Environmental Level.}\\ At the environmental level, the attacker has knowledge of the approximate position of the target object, allowing them to define a frustum region for placing spoofed points. This information not only enables false positive outcomes but also makes it possible to launch false negative or translation attacks, which target specific legitimate objects within the scene.

%%==============================================
\subsubsection{Attack Goal}
%%==============================================

\textbf{Object Injection or false positive (FP) outcome}: The goal of the adversary in object injection attacks is to cause the model to generate redundant bounding boxes or to detect and classify nonexistent objects within the input image. By injecting these false objects into the model's perception, the attacker aims to deceive the system into recognizing and responding to entities that are not actually present in the environment, potentially leading to erroneous decisions by the autonomous vehicle, such as unnecessary evasive maneuvers or incorrect navigation. %The adversary can learn δ to increase objectness scores of candidate boxes.

The goal of achieving a false positive outcome is to force the victim to perform dangerous maneuvers (e.g., emergency braking or lane change) to avoid the false object. For example, LiDAR spoofing attacks can result in safety-critical incidents, as shown with Baidu’s Apollo \cite{Baidu, sun2020}.

\noindent\textbf{Object Removal or false negative (FN) outcome}: The goal of the adversary in object removal attacks is to cause the model to miss detecting objects that are actually present in the environment. By manipulating the input data or the physical environment, the attacker aims to prevent the model from recognizing certain objects, effectively erasing them from the system’s perception. This can lead to dangerous situations, as the autonomous vehicle may fail to respond appropriately to obstacles, pedestrians, or other critical objects, increasing the risk of accidents.

The goal of achieving a false negative outcome is to remove an existing object from the perception output such that path planning and control are compromised. Such attacks can have the devastating consequence of the victim crashing into an unsuspecting object hidden to perception (e.g., as in \cite{cao2021}).

\noindent\textbf{Translation}: FP and FN outcomes are insufficient to fully capture the effects of perception attacks. Some cascaded semantic fusion architectures (e.g., FPN) enforce one-to-one matching between 2D and 3D detections; thus, an FP necessarily implies an FN. We call such instances translation outcomes as the attacker has created physical distance between the negated ground truth (FN) and the spoofed detection (FP). Translation outcomes may cause emergency braking if objects are moved to front-near positions or collision when moved farther from the victim or to a different lane.

\noindent\textbf{Miscategorization}: The goal of the adversary in miscategorization attacks is to perturb the input data in a way that causes the model to predict an incorrect label for a detected object.

% \noindent\textbf{System Disruption}: The overall goal may be to cause the system to behave unpredictably, leading to navigation errors or unsafe decisions.
%==========================
\subsection{Attack method}
%==========================
\label{method}
\subsubsection{Detector Type}
% 3D object detection plays an important role in the field of autonomous driving and has rapid development benefited from the breakthroughs in deep learning and sensor technologies.
\noindent\textbf{Single-Sensor Models}: Understanding the environment in 3D provides autonomous vehicles (AVs) with more comprehensive and reliable information compared to using 2D bounding boxes or pixel masks. With the growing adoption of 3D sensors, it's now possible to capture and process larger volumes of 3D data, delivering accurate depth information crucial for both mobile devices and AVs. Point clouds, which capture the 3D coordinates of points sampled from the surfaces of physical or virtual objects, are a widely used data format in 3D vision applications such as industrial modeling, surveying, and autonomous driving. Unlike images that consist of ordered pixels, point clouds are unordered, making them challenging to analyze using conventional deep learning techniques. To address these challenges, several methods have been developed to design deep learning models capable of processing point cloud data for tasks like classification and object detection. These methods can be broadly categorized into three types: Voxel-based approaches, Bird's-eye view techniques, and PointNet-based methods.

%\noindent\textit{\textbf{Voxel-based architecture}} VoxelNet \cite{zhou2018voxelnet} divides the point cloud into equally-spaced 3D voxels, allowing for ordered analysis. Then 3D Convolutional Neural Networks (CNNs) are applied for 3D bounding box prediction, after which a 2D convolutional detection layer is applied in the final stage. Many recent works \cite{lehner2019patch, kuang2020voxel, yan2018second} adopt this voxel-based architecture and achieve state-of-the-art performance. PointPillar \cite{lang2019pointpillars}, is another example of a voxel-based method. It utilizes an encoder to convert features learned from voxelized point clouds into sparse pseudo images. The final predictions are given by applying 2D CNNs and a SSD-based \cite{Liu_2016} detection network on the pseudo images. 
\noindent\textit{- \textbf{Voxel-based Architecture.}} VoxelNet \cite{zhou2018voxelnet} organizes point clouds into uniformly spaced 3D voxels, enabling structured analysis. This method applies 3D Convolutional Neural Networks (CNNs) for predicting 3D bounding boxes, followed by a 2D convolutional detection layer in the final stage. Several recent studies \cite{lehner2019patch, kuang2020voxel, yan2018second} have adopted this voxel-based approach, achieving state-of-the-art results. PointPillar \cite{lang2019pointpillars} is another example of a voxel-based technique. It employs an encoder to transform features extracted from voxelized point clouds into sparse pseudo-images, with final predictions made by applying 2D CNNs and an SSD-based \cite{Liu_2016} detection network on these pseudo-images.

% \noindent\textit{\textbf{Bird-eye view architecture}}
% Using Deep Neural Networks (DNN) to process 2D images is a mature technique and as such, researchers transform LiDAR point clouds into ordered 2D structures for 3D object detection in AV systems. These methods \cite{chen2017multi, shi2020pv, yang2018pixor} convert the point cloud to a bird’s eye view representation for efficiency and exploits 2D convolutions. PV-RCNN \cite{shi2020pv} as one target model in the black-box setting since it achieves high performance in the KITTI bird’s eye view benchmark.
% MV3D \cite{chen2017multi}
% Pixor \cite{yang2018pixor}
\noindent\textit{- \textbf{Bird's-Eye View Architecture.}}  
Leveraging Deep Neural Networks (DNNs) to process 2D images is a well-established technique. Consequently, researchers have developed methods to convert LiDAR point clouds into ordered 2D structures for 3D object detection in autonomous vehicle (AV) systems. These approaches \cite{shi2020pv, yang2018pixor} transform the point cloud data into a bird's-eye view representation, which allows for more efficient processing using 2D convolutions. For instance, PV-RCNN \cite{shi2020pv}, known for its high performance in the KITTI bird's-eye view benchmark, is often used as a target model in black-box attack scenarios. Other notable examples of this approach include PIXOR \cite{yang2018pixor}.

% \noindent\textit{\textbf{PointNet-based architecture}}
% Bird-eye and voxel based methods apply deep learning models to analyze point cloud data by decreasing computation cost and improving performance with sparse data. However, these methods cannot directly process raw point cloud data and instead rely on transformation techniques to convert the raw point cloud data into a form that can be easily processed. Though easy to operate, the performance of these schemes is limited by information loss. In comparison, PointNet \cite{qi2017pointnet} and PointNet++ \cite{qi2017pointnet++} apply max-pooling and transformations to reduce the unordered and dimensionally flexible input data to fixed-length global feature vectors. By doing so, they enable end-to-end neural network learning architectures on raw point cloud data. PointNet demonstrates its robustness by introducing the concept of critical points and upper bounds. PointNets are widely adopted in different applications such as 3D object detection \cite{shi2019pointrcnn, qi2018frustum} as backbone feature generation networks. 
\noindent\textit{- \textbf{PointNet-Based Architecture.}}  
Bird's-eye view and voxel-based methods utilize deep learning models to analyze point cloud data, aiming to reduce computational costs and improve performance with sparse data. However, these methods cannot process raw point cloud data directly and instead require transformation techniques to convert the raw data into a more structured form that can be easily processed. While these transformations simplify the processing, they often lead to some degree of information loss, limiting the overall performance. In contrast, PointNet \cite{qi2017pointnet} and PointNet++ \cite{qi2017pointnet++} are designed to handle raw point cloud data directly by applying max-pooling and transformations to convert the unordered and dimensionally flexible input data into fixed-length global feature vectors. This approach enables end-to-end learning architectures on raw point cloud data, preserving more of the original information. PointNet is particularly robust due to its introduction of critical points and upper bounds concepts. PointNets are widely used in various applications, including 3D object detection \cite{shi2019pointrcnn, qi2018frustum}, where they serve as backbone networks for feature extraction.

%=================================================
% \subsection{Sensor-fusion 3D Object Detection }
% \textbf{Integration with other sensors (sensor fusion)}
%=================================================

% \cite{liu2021}
% In order to improve the robustness of the models and enhance the perception, sensor-fusion 3D object detection methods have been proposed which leverage multiple types of sensors with complementary characteristics. Due to the complementary and shared information, the fusion of multiple sensors is considered to achieve higher accuracy and stronger robustness in detection tasks than single sensor. AVs are safety-critical applications and the reliability of object detectors is important, therefore, they frequently utilize the fusion detection models of LiDAR and camera, with the advantages of depth information provided by point clouds and texture information captured by images. According to the different levels of fusion, multi-modal fusion can be divided into three major streams: early fusion (input level), deep fusion (feature level) and late fusion (decision level). 
\noindent\textbf{Multi-Sensor Fusion Models}: To enhance the robustness of models and improve perception capabilities, sensor-fusion 3D object detection methods have been developed, leveraging multiple types of sensors with complementary characteristics. By integrating the unique strengths of different sensors, such as the depth information from LiDAR point clouds and the texture details from camera images, sensor fusion is recognized for achieving higher accuracy and greater robustness in detection tasks compared to using a single sensor alone. Given that autonomous vehicles are safety-critical systems, the reliability of object detectors is paramount. As a result, AVs often employ fusion detection models that combine data from both LiDAR and cameras, capitalizing on the complementary nature of these sensors. Based on the stage at which fusion occurs, multi-sensor fusion can be categorized into two main approaches: Cascaded Fusion and Parallel Fusion.

% Cascaded Fusion: Frustum-based, and Painting-based

In cascaded fusion, the integration of sensor data occurs in a sequential manner. Typically, one sensor's data, such as the camera's visual information, is processed first to identify key features or regions of interest. This processed data is then used to guide or refine the interpretation of the second sensor's data, like LiDAR, which provides depth and spatial information. The cascaded approach leverages the strengths of each sensor in stages, where the initial sensor can help focus or improve the accuracy of subsequent data interpretation. This method is beneficial for refining detections and reducing the computational load by narrowing down the areas for LiDAR analysis based on camera data.

PointFusion \cite{xu2018pointfusion} first processes the camera images to extract 2D region proposals. These proposals are then used to guide the processing of LiDAR point clouds. The 3D points are extracted only within the regions of interest (ROIs) identified by the camera, which reduces computational complexity. It allows the system to focus on specific areas identified as potential objects by the camera, making the subsequent LiDAR processing more efficient.

MV3D (Multi-View 3D) \cite{chen2017multi} employs a cascaded fusion technique where it first uses 2D region proposals from camera images and then combines these proposals with LiDAR point clouds to generate 3D bounding boxes. The fusion occurs by projecting the 3D proposals onto bird's-eye view and front view for refinement. This method capitalizes on the strengths of both sensors by using camera data to guide the extraction of regions of interest from LiDAR data, improving 3D localization accuracy. %Chen et al. \cite{chen2017multi} introduced the MV3D approach, which generates 3D region proposals using a proposal network based on the bird’s-eye view (BEV) representation of LiDAR point cloud data. These proposals are then projected onto multiple views, and the region-wise BEV features are fused with camera image features extracted from a multi-branch representation network.

% Parallel Fusion:
Parallel fusion involves processing and integrating data from both LiDAR and cameras simultaneously. In this approach, the data from both sensors are processed in parallel, with each contributing its unique information to a unified perception model. The integration is done at a later stage, combining the spatial and texture information from LiDAR and camera data to produce a more robust and comprehensive understanding of the environment. Parallel fusion allows for a more holistic approach to perception, as it can consider the full data set from both sensors simultaneously, enhancing the system’s ability to detect and classify objects accurately in various conditions.

%Parallel Fusion: Early-Fusion, Middle-Fusion, Late-Fusion, and Mixed-Fusion.
%Parallel Fusion: Input-Level Fusion (Early Fusion), Feature-Level Fusion (Deep Fusion), and Decision-Level Fusion (Late Fusion).

\noindent\textit{\textbf{Input-Level Fusion (Early Fusion)}} is fusing data from multiple sensors right at the beginning of the processing pipeline before any significant feature extraction or processing takes place. This approach integrates different types of raw data early on, allowing the model to process and learn from this combined input throughout its layers.

% \noindent\textit{\textbf{Feature-Level Fusion (Deep Fusion)}} is fusing the features extracted from point cloud data and image data through a certain stratege (e.g. addition, mean, concatenation), and then feed it into detection network to obtain the final detection results, e.g. MV3D \cite{chen2017multi}, AVOD \cite{ku2018joint}, EPNet \cite{huang2020epnet}. 

% Chen et al. \cite{chen2017multi} propose a MV3D approach which uses a proposal network to generate 3D region proposals from the bird’s eye view (BEV) representation of LiDAR point cloud data and projects them to multiple views. Then it fuses the region-wise BEV and camera image features generated from multi-branch representation network. Qi et al. \cite{8578200} propose a cascading approach F-PointNet, which first produces 2D proposals from camera images and projects them to the LiDAR view as frustum proposals. The LiDAR point clouds in the frustum proposals are then used to generates corresponding 3D boxes. Vora et al. \cite{vora2020pointpainting} propose a PointPainting method which projects LiDAR point clouds into the output of an image-only semantic segmentation network and appends the segmentation scores to each point. Then the painted point clouds can be fed to a LiDAR-only detector for 3D object detection. Huang et al. \cite{huang2020epnet} propose an EPNet which fuses the features of LiDAR point clouds and camera images in a point-wise manner and uses a consistency enforcing loss to solve the issue of the inconsistency between the classification confidence and localization confidence. The EPNet model produces the state-of-the-art sensor-fusion based 3D object detection performance. AVOD \cite{ku2018joint} a typical two-stage object detection architecture with a region proposal network (RPN) and a second stage detection network. It uses feature extractors to generate feature maps from point clouds and images which are then shared by two sub-networks. First the feature maps are fed into RPN and fused via an element-wise mean operation after cropping and resizing, and then generate top k proposals through fully connected layers. Second projecting the proposals on feature maps and adopting similar fusion operations in RPN stage to generate final detections, including box regression, orientation estimation and category classification. In MVX-Net (Multi-View Fusion Network) \cite{sindagi2019mvx}, the point cloud data is first voxelized, and then a 3D convolutional neural network (CNN) is used to extract features from the voxelized point cloud. Features are extracted from the RGB images using a standard 2D CNN, which processes the image to identify key visual features such as edges, textures, and colors. After independent feature extraction from the LiDAR and camera data, the model fuses these features at a deep level in the network. This involves aligning the features from the two modalities in a way that they can be combined effectively. The fusion process typically involves projecting the 3D LiDAR features into the 2D image space or vice versa, aligning the features based on spatial correspondences between the LiDAR points and image pixels.

\noindent\textit{\textbf{Feature-Level Fusion (Deep Fusion)}} involves combining features extracted from different sensor modalities, such as point cloud data and image data, through various strategies (e.g., addition, averaging, or concatenation). These fused features are then fed into a detection network to obtain the final detection results. Examples of models that utilize this approach include AVOD \cite{ku2018joint}, and EPNet \cite{huang2020epnet}.

Qi et al. \cite{8578200} proposed F-PointNet, a cascading approach that first produces 2D proposals from camera images and projects them onto the LiDAR view as frustum proposals. The LiDAR point clouds within these frustum proposals are then used to generate corresponding 3D bounding boxes. Vora et al. \cite{vora2020pointpainting} introduced the PointPainting method, where LiDAR point clouds are projected into the output of an image-only semantic segmentation network. The segmentation scores are appended to each point, and the "painted" point clouds are subsequently fed into a LiDAR-only detector for 3D object detection. Huang et al. \cite{huang2020epnet} developed EPNet, which fuses the features of LiDAR point clouds and camera images on a point-wise basis. EPNet also introduces a consistency enforcing loss to address the inconsistency between classification confidence and localization accuracy, resulting in state-of-the-art performance for sensor-fusion-based 3D object detection. AVOD \cite{ku2018joint} employs a typical two-stage object detection architecture with a Region Proposal Network (RPN) followed by a second-stage detection network. It uses feature extractors to generate feature maps from both point clouds and images, which are then shared by two sub-networks. Initially, the feature maps are fed into the RPN and fused via an element-wise mean operation after cropping and resizing, generating the top k proposals through fully connected layers. These proposals are then projected onto the feature maps, where similar fusion operations as in the RPN stage are applied to produce the final detections, including box regression, orientation estimation, and category classification. In MVX-Net (Multi-View Fusion Network) \cite{sindagi2019mvx}, the point cloud data is first voxelized, and a 3D convolutional neural network (CNN) is used to extract features from the voxelized point cloud. Simultaneously, features are extracted from RGB images using a standard 2D CNN to identify key visual characteristics such as edges, textures, and colors. After independent feature extraction from the LiDAR and camera data, these features are fused at a deep level within the network. This fusion process typically involves projecting the 3D LiDAR features into the 2D image space, or vice versa, aligning the features based on spatial correspondences between the LiDAR points and image pixels, effectively combining the information from both modalities.

% \noindent\textit{\textbf{Decision-Level Fusion (Late Fusion)}} is fusing the results detected by LiDAR perception network and camera perception network respectively through a certain rule (e.g. geometric association, semantic consistency), e.g. CLOCs \cite{pang2020clocs}, models designed in Apollo \cite{apollo} and Autoware \cite{autoware}. CLOC \cite{pang2020clocs} (Camera-LiDAR Object Candidates) is a model designed for 3D object detection in autonomous vehicles, specifically focusing on combining (or fusing) object detection results from both camera and LiDAR modalities at a decision level. CLOC stands for Camera-LiDAR Object Candidates Fusion, and it represents a form of late fusion in the context of multi-modal data processing. CLOC begins by performing object detection independently on the camera and LiDAR data. Typically, a 2D object detector (such as Faster R-CNN) processes the camera images to generate 2D bounding boxes, while a separate 3D object detector processes the LiDAR point cloud to generate 3D bounding boxes.
\noindent\textit{\textbf{Decision-Level Fusion (Late Fusion)}} refers to the process of combining the results from separate detection networks, such as those based on LiDAR and camera data, after each modality has independently processed its input. The fusion occurs at the decision-making stage, where the outputs from both networks are merged using specific rules, such as geometric association or semantic consistency. This approach is exemplified by models like CLOCs \cite{pang2020clocs} and systems implemented in platforms like Apollo \cite{apollo} and Autoware \cite{autoware}. CLOC \cite{pang2020clocs} (Camera-LiDAR Object Candidates) is a model specifically designed for 3D object detection in autonomous vehicles, utilizing decision-level fusion to integrate object detection results from both camera and LiDAR modalities. In this approach, object detection is first performed independently on camera and LiDAR data. Typically, a 2D object detector (such as Faster R-CNN) processes the camera images to generate 2D bounding boxes, while a separate 3D object detector processes the LiDAR point cloud to generate 3D bounding boxes. The results from these independent detectors are then fused at the decision level, combining the strengths of both modalities to enhance the overall detection accuracy and robustness.


% \begin{table*}
%     \centering
%     \begin{tabular}{ccc}
%     \toprule
%      \textbf{Modality}    & \textbf{Detector type} & \textbf{Model/algorithm}\\
%      \midrule
%          & Voxel-based architecture& VoxelNet \cite{zhou2018voxelnet}, PointPillar \cite{lang2019pointpillars}\\
%       Single-modality models   & Bird’s-Eye View architecture &PV-RCNN \cite{shi2020pv}, PIXOR \cite{yang2018pixor}\\
%       (LiDAR-only)                  & PointNet-Based architecture& PointNet \cite{qi2017pointnet}, PointNet++ \cite{qi2017pointnet++}, PointRCNN, Point-GNN\\
%                         & Input-Level Fusion & \\
%       Multi-modality models    & Feature-Level Fusion & MV3D \cite{chen2017multi}, AVOD \cite{ku2018joint}, EPNet \cite{huang2020epnet}, \\
%        (Multi-modal fusion)       &          &  PointPainting \cite{vora2020pointpainting}, F-PN \cite{8578200}, MVX-Net \cite{sindagi2019mvx}   \\
%                        & Decision-Level Fusion & CLOC \cite{pang2020clocs}\\
%     \bottomrule
%     \end{tabular}
%     \caption{Models used in literature to evaluate adversarial attacks for 3D object detection.}
%     \label{tab:detectors}
% \end{table*}

% \textcolor{red}{other categorization}

% Cascaded semantic-level fusion (Frust. -ConvNet, Frust. -PointNet )
% Integrated semantic-level fusion (Baido Apollo)
% Feature-level fusion (AVOD, EPNET)

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{Figures/fusion_level.png}
%     \caption{ (Figure adapted from \cite{hallyburton2022}).}
%     \label{fig:fusion_level}
% \end{figure*}
% \textcolor{red}{fusion-based vs. cascaded}

\subsubsection{Attack Form}

% \cite{Sato2023}
% Due to the basic sensing mechanism of laser firing and receiving, LiDARs are fundamentally vulnerable to malicious laser shooting, or LiDAR spoofing attacks. Specifically, such attacks work by using an external attack device (“spoofer”) to fire laser pulses back to the victim LiDAR in order to manipulate the time measurements of the laser-receiving events and thus the corresponding 3D position measurements (§II-A).
% Such point position manipulations can thus be strategically used to achieve attack effects on the 3D object detector side, more specifically (1) Object injection, e.g., by moving the positions of a set of points to form a 3D pattern to cause a false-positive detection of a non-existing object; and (2) Object removal, e.g., by moving the points originally on an object to elsewhere to cause false-negative detection of such an object.

% \textbf{Sensor-level spoofing} 
% Spoofing attacks involve injecting fake or manipulated LiDAR signals to create phantom objects or alter the perception of real objects. This can confuse the autonomous vehicle’s decision-making process by presenting false data.

% The impact of these spoofing attacks includes the creation of non-existent obstacles, which can force unnecessary evasive maneuvers, and manipulation of the perceived environment, leading to incorrect navigation and potential collisions.

\noindent\textbf{Spoofing Attacks}: Sensor spoofing attacks use the same physical channels as the targeted sensor to manipulate the sensor readings.  The adversary can achieve this by deploying a device within the line of sight of a victim vehicle’s LiDAR sensor. The adversarial device can capture LiDAR signals, alter them and emit them toward the victim sensor with a controlled delay. By controlling the return signal, the attacker can manipulate the resulting 3D measurements reported in a 3D point cloud by the victim sensor. This strategy makes it very difficult for the sensor system to recognize such attack, since the attack doesn’t require any physical contact or tampering with the sensor, and it doesn’t interfere with the processing and transmission of the digital sensor measurement. These types of attack could trick the victim sensor to provide seemingly legitimate but actually erroneous data. \cite{cao2019ccs}

% Signal interference attacks involve emitting signals that interfere with the LiDAR system’s operation, either by introducing noise or by creating misleading signals that confuse the sensor. These attacks can effectively blind or mislead the LiDAR system, compromising the vehicle's perception and navigation capabilities.

% The attacks involve subtle modifications to the environment or objects within the LiDAR sensor's field of view to cause misclassification or non-detection. These attacks aim to deceive the perception algorithms without being easily noticeable.

% Designing objects with specific shapes or materials that disrupt the LiDAR signal reflection, leading to incorrect interpretations.

% The impact of these evasion attacks is profound, as they can result in the failure to detect critical objects, such as pedestrians or other vehicles, and incorrect classification of objects, potentially leading to unsafe decisions.


% \noindent\textbf{Physical Adversarial Objects}: Physical adversarial examples involve modifying the physical environment or objects within the LiDAR sensor’s field of view to create misleading point clouds, causing misclassification or non-detection of objects. 
% Designing objects with specific shapes or materials that disrupt the LiDAR signal reflection, leading to incorrect interpretations.
\noindent\textbf{Physical Adversarial Objects:}  
These attacks involve designing physical objects with carefully crafted shapes that, when placed within the LiDAR sensor’s field of view, disrupt signal reflection. This manipulation results in misleading point clouds, which can cause the system to either misclassify or completely fail to detect objects. The adversarial objects are specifically designed to exploit weaknesses in the perception algorithms, making them appear as normal, yet altering the sensor's interpretation of the environment in critical ways.

\noindent\textbf{Reflective Objects}: Reflective objects can introduce errors in LiDAR perception by creating false or distorted point cloud data. Highly reflective surfaces, such as mirrors or polished metal, can reflect LiDAR signals in unexpected ways, leading to incorrect distance measurements or even ghost objects appearing in the LiDAR’s point cloud. These reflective materials can be strategically placed in an adversarial manner to disrupt the sensor’s ability to accurately perceive its surroundings.
%==============================================
\subsubsection{Placement in Physical Space}
%==============================================

\textbf{In Physical Proximity}: Locality in physical space refers to the necessity of an adversary being in close physical proximity to the target in order to carry out certain types of attacks. For many physical attacks, such as those involving direct manipulation of the environment or objects within the LiDAR sensor's field of view, the attacker must be near the target vehicle or sensor system. This proximity allows the attacker to place or alter objects, introduce reflective materials, or otherwise influence the physical environment in ways that the LiDAR system will misinterpret.

%\textbf{On the Target Objects}: In addition to being in proximity, the attacker may need to focus specifically on the target objects themselves. This could involve attaching physical adversarial examples, such as stickers or coverings, directly to the objects that the LiDAR is intended to detect. By being able to manipulate these target objects, the adversary can ensure that the LiDAR system misclassifies or fails to detect them, thereby achieving the desired adversarial effect. This kind of localized attack requires precision and often direct interaction with the objects of interest in the physical environment.
\noindent\textbf{On the Target Objects}: In addition to being in proximity, the attacker may need to focus specifically on the target objects themselves. This could involve adding a physical adversarial object on top of a target object, subtly altering its appearance or characteristics.


